Optimal Non-Oblivious Open Addressing

A hash table is said to be open-addressed (or non-obliviously open-addressed) if it stores elements (and free slots) in an array with no additional metadata. Intuitively, open-addressed hash tables must incur a space-time tradeoff: The higher the load factor at which the hash table operates, the longer insertions/deletions/queries should take. In this paper, we show that no such tradeoff exists: It is possible to construct an open-addressed hash table that supports constant-time operations even when the hash table is entirely full. In fact, it is even possible to construct a version of this data structure that: (1) is dynamically resized so that the number of slots in memory that it uses, at any given moment, is the same as the number of elements it contains; (2) supports $O(1)$-time operations, not just in expectation, but with high probability; and (3) requires external access to just $O(1)$ hash functions that are each just $O(1)$-wise independent. Our results complement a recent lower bound by Bender, Kuszmaul, and Zhou showing that oblivious open-addressed hash tables must incur $\Omega(\log \log \varepsilon^{-1})$-time operations. The hash tables in this paper are non-oblivious, which is why they are able to bypass the previous lower bound.

==> techoverview.tex <==
We formalize the task of implementing a RAM in the open-addressing model as follows. The RAM is a sequence of machine words $v_1, \ldots, v_m$, each is an integer in $[2^w]$ as the word-size $w = \Theta(\log n)$. We denote by $M = m \cdot w$ the total number of bits in the RAM. We need to support the following \emph{RAM operations}:
\begin{itemize}
\item RAM reads: given a word-index $i$, return the value $v_i$ of the $i$-th machine word.
\item RAM writes: given a word-index $i$ and a value $v_i^*$, update the value of the $i$-th machine word to $v_i^*$.
\end{itemize}
The purpose of this section is to develop intuition of encoding information by permuting the keys via a toy example: Assume we have a set $S$ of $n$ keys and a perfect hash function $f$ that maps all keys to different slots, we are going to encode an $O(n \log n)$-bit RAM, such that RAM reads and writes are performed within $O(1)$ probes to the slots in expectation.

We first store all keys in the slots indicated by $f$, i.e., we store each key $x \in S$ in the slot $f(x)$. When we allow key $x$ to be stored in a different slot than $f(x)$, the hash value $f(x)$ serves as a \emph{pointer}. Formally, for every key $x$ stored in a slot $i$, we think its pointer $P(x)$ is pointing at the key stored in the $f(x)$-th slot. When $x$ is stored at slot $f(x)$ at the beginning, the pointer $P(x) = x$, in which case we call $x$ a \emph{self-loop}.

For two self-loops $x$ and $y$ stored at slots $f(x)$ and $f(y)$ respectively, we can swap their locations such that $f(x) = y$, $f(y) = x$, i.e., their pointers form a cycle of length 2. In this case, we say $x$ and $y$ form a \emph{pair}. Given a key, it is very easy to detect if it is in a pair, and if so, to reach its partner. When the pair is formed, $x$ is physically stored at $f(y)$, but we still view $f(x)$ as its ``logical address'', and say $f(y)$ is its ``physical address''.

For a fixed self-loop $x$ at the beginning, it can form pairs with numerous keys, so we may encode information using the choice of partner. Formally, we call the first $0.1n$ slots the \emph{index slots}, and divide the remaining $0.9n$ slots into $\sqrt n$ regions of equal sizes, each consisting of $0.9 \sqrt n$ slots. For the key $x_i$ that was hashed to the $i$-th index slot, we encode the $i$-th machine word $v_i$: assuming $v_i \in [\sqrt n]$ ($w = \frac{1}{2} \log n$), we arbitrarily pick a self-loop key $y$ in the $v_i$-th region, and let it form a pair with $x_i$. Thus, in order to read the $i$-th machine word, we only need to probe the $i$-th index slot, and return the region ID which the destination of pointer belongs to.

To write or update the $i$-th word in the RAM, we first break the formed pair involving $x_i$ (if exists), and then let $x_i$ pair with an arbitrary self-loop in the target region. This is $O(1)$ expected time as long as at least $\Omega(1)$ fraction of slots in that region are self-loops, which holds on average over all regions. To avoid running out of self-loops in a given region, we randomly shift the machine-word values $v_i$ to $v'_i \defeq v_i \oplus r_i$, where $r_i$ are independently uniformly random numbers that are fixed over time. That is, to encode a machine word $v_i$, we actually let $x_i$ pair with a self-loop key in the $v'_i$-th region. By Chernoff bounds, we know that with $\ge 1 - n^{-100}$ probability, for every region $k$, the ``demand'' of self loops in the $k$-th region $|\BK{i \in [0.1n] : v'_i = k}| \le 0.2 \sqrt n$, which means more than half of the slots in that region will contain self-loops.

Moreover, this framework also supports \emph{key operations}. As every key only appears in a self-loop or a pair, key queries are completed within 2 slot-probes: either $x$ is directly stored at the $f(x)$-th slot, or $y$ is stored in that slot while $x$ is stored in $f(y)$. Similarly, we can perform one deletion followed by one insertion, as long as $f$ is still a perfect hash function for the set of keys: we may de-pair all slots involved in the operation, and perform key operations straightforwardly; after the operations are done, we pair back these keys again. The time complexity is still $O(1)$.

